Representing 3D Shapes With 64 Latent Vectors for 3D Diffusion Models

Constructing a compressed latent space through a variational autoencoder (VAE) is the key for efficient 3D diffusion models. This paper introduces COD-VAE that encodes 3D shapes into a COmpact set of 1D latent vectors without sacrificing quality. COD-VAE introduces a two-stage autoencoder scheme to improve compression and decoding efficiency. First, our encoder block progressively compresses point clouds into compact latent vectors via intermediate point patches. Second, our triplane-based decoder reconstructs dense triplanes from latent vectors instead of directly decoding neural fields, significantly reducing computational overhead of neural fields decoding. Finally, we propose uncertainty-guided token pruning, which allocates resources adaptively by skipping computations in simpler regions and improves the decoder efficiency. Experimental results demonstrate that COD-VAE achieves 16x compression compared to the baseline while maintaining quality. This enables 20.8x speedup in generation, highlighting that a large number of latent vectors is not a prerequisite for high-quality reconstruction and generation. The code is available at https://github.com/join16/COD-VAE.

==> Main/Partials/figure_method_vecset.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{Main/Assets/figure_vecset.pdf}
    \vspace{-15pt}
    \caption{Visualization of latent vectors of VecSet.}
    \label{fig:method_vecset}
    \vspace{-10pt}
\end{figure}

==> Supple/Partials/table_extra_gen.tex <==
\begin{table}[]
    \setlength{\tabcolsep}{6pt}
    \centering
    \footnotesize
    \begin{tabular}{c|cc|cc|cc|cc}
    \toprule
    \multirow{2}{*}{Method} & \multirow{2}{*}{Rendering-FID $\downarrow$} & \multirow{2}{*}{Surface-FPD $\downarrow$} & \multicolumn{2}{c}{MMD $\downarrow$} & \multicolumn{2}{c}{COV (\%) $\uparrow$} & \multicolumn{2}{c}{1-NNA (\%) $\downarrow$} \\
      % & CD ($\times 10^3$) & EMD ($\times 10^2$) & CD & EMD & CD & EMD & & & Diffusion & Full  \\
        & &  & CD & EMD & CD & EMD & CD & EMD \\
    \hline
    
    SDF-StyleGAN~\cite{zheng2022sdf}    & 73.66	& 1.43	& 5.59	& 10.81	& 72.72	& 70.03	& 57.87	& 58.88 \\
    LAS-Diffusion~\cite{zheng2023las}   & 45.98	& 0.64	& 4.52	& 9.80	& 77.96	& 78.46	& 52.91	& 51.87 \\
    Octfusion~\cite{xiong2024octfusion}       & -     & -     & -     & -     & -     & -     & -     & - \\ \hline
    3DILG \cite{zhang20223dilg} & 64.83 & 2.585 & 6.270 & 10.98 & 58.16 & 62.80 & 61.49 & 59.90 & 0.14 & 0.09 \\
    GEM3D \cite{petrov2024gem3d} & 47.98 & 0.997 & 5.381 & 10.41 & 66.64 & 66.05 & 54.74 & 56.02 & 0.09 & 0.07 \\ 
    VecSet ($M=32$) \cite{zhang2023vecset} & 65.56 & 0.800 & 4.999 & 10.44 & 84.51 & 82.85 & 54.32 & 54.76 & 39.77 & 2.81 \\
    VecSet ($M=64$) & 54.47 & 0.629 & 5.090 & 10.49 & 84.89 & 84.45 & 55.04 & 54.94 & 21.92 & 2.63 \\
    VecSet ($M=512$) & 44.18 & 0.521 & \textbf{4.807} & \textbf{10.21} & 85.20 & 84.23 & 53.78 & 55.06 & 2.59 & 1.16 \\ 
    Ours ($M=32$) & 37.34 & 0.473 & 5.020 & 10.38 & 84.96 & 84.23 & \textbf{53.11} & 54.09 & \textbf{41.19} & \textbf{24.17}\\
    Ours ($M=64$) & \textbf{37.05} & \textbf{0.460} & 5.025 & 10.38 & \textbf{86.03} & \textbf{85.37} & 54.89 & \textbf{54.07} & 22.49 & 16.09 \\
    \bottomrule
    
    \end{tabular}
    \vspace{-5pt}
    \caption{
    \textbf{Class-conditioned generation results on ShapeNet.}
    The scales of MMD are $10^{-3}$, and $10^{-2}$ for CD, and EMD, respectively.
    % The throughput is measured using a single A6000 GPU with a batch size 64. 
    }
    \label{table:shapenet_gen}
    \vspace{-10pt}
\end{table}
